Histo-Diffusion: A Diffusion Super-Resolution Method for Digital Pathology with Comprehensive Quality Assessment

Digital pathology has advanced significantly over the last decade, with Whole Slide Images (WSIs) encompassing vast amounts of data essential for accurate disease diagnosis. High-resolution WSIs are essential for precise diagnosis but technical limitations in scanning equipment and variablity in slide preparation can hinder obtaining these images. Super-resolution techniques can enhance low-resolution images; while Generative Adversarial Networks (GANs) have been effective in natural image super-resolution tasks, they often struggle with histopathology due to overfitting and mode collapse. Traditional evaluation metrics fall short in assessing the complex characteristics of histopathology images, necessitating robust histology-specific evaluation methods. We introduce Histo-Diffusion, a novel diffusion-based method specially designed for generating and evaluating super-resolution images in digital pathology. It includes a restoration module for histopathology prior and a controllable diffusion module for generating high-quality images. We have curated two histopathology datasets and proposed a comprehensive evaluation strategy which incorporates both full-reference and no-reference metrics to thoroughly assess the quality of digital pathology images. Comparative analyses on multiple datasets with state-of-the-art methods reveal that Histo-Diffusion outperforms GANs. Our method offers a versatile solution for histopathology image super-resolution, capable of handling multi-resolution generation from varied input sizes, providing valuable support in diagnostic processes.

==> table_0611.tex <==
\begin{table*}[t]\small
\centering
\caption{ Comparison with state-of-the-art GAN-based and Diffusion based methods on histopathology image datasets with a 4× upsampling scale on PRAD-100, LUAD-100, GBM-100 dataset using our proposed metrics.  The best and second best results are highlighted in \textbf{bold} and \underline{underline}. }
\label{table1}
\resizebox{0.7\textwidth}{!}{%
\begin{tabular}{c|c|c|c c c c c}
\hline
\multirow{2}{*}{Datasets} &\multirow{2}{*}{Methods} &\multirow{2}{*}{Scale} & \multicolumn{4}{c}{Metrics}\\ \cline{4-8}
 & & & & $L1_{texture}\downarrow$ & $L1_{intensity}\downarrow$ & CLIPIQA (boxblur)$\uparrow$ & CLIPIQA (Gaussian) $\uparrow$ \\ \hline
 \hline

\multirow{5}{*}{PRAD-100} & Bicubic& $\times4$ & &\underline{274.21}&\underline{14.74}&0.8109 &0.8197\\
 &BSRGAN& $\times4$ & &348.65&20.77&0.9015&0.8776\\ 
 &Real-ESRGAN& $\times4$ & &321.15&15.38&0.8884&0.8974\\ 
 &SwinIR-GAN& $\times4$ & &321.94&15.14&\underline{0.9304}&\underline{0.9288}\\\cline{2-8}
 &Ours& $\times4$ & &\textbf{224.95}&\textbf{11.83}&\textbf{0.9468}&\textbf{0.9458}\\\hline 
 \hline

\multirow{5}{*}{LUAD-100} & Bicubic& $\times4$ & &\underline{236.01}&\textbf{15.26}&0.8768&0.8943 \\
 &BSRGAN& $\times4$ & &247.74&19.07&0.9010&0.8934\\ 
 &Real-ESRGAN& $\times4$ & & 159.72&11.81&\underline{0.9359}&\underline{0.9364}\\ 
 &SwinIR-GAN& $\times4$ & & 193.39&12.55&0.9307&0.9355\\\cline{2-8}
 &Ours& $\times4$ & &\textbf{200.70}&\underline{12.83}&\textbf{0.9497}&\textbf{0.9504}\\\hline 
 \hline
 
\multirow{5}{*}{GBM-100} & Bicubic& $\times4$ & &\underline{636.75}&\underline{30.99}&0.7784 &0.7566\\
 &BSRGAN& $\times4$ & &741.62&37.17&0.9245&0.8965\\ 
 &Real-ESRGAN& $\times4$ & & 682.92&28.89&0.9032&0.9026\\ 
 &SwinIR-GAN& $\times4$ & & 723.11&29.96&\underline{0.9419}&\underline{0.9276}\\\cline{2-8}
 &Ours& $\times4$ & &\textbf{639.70}&\textbf{28.10}&\textbf{0.9513}&\textbf{0.9343}\\\hline 
 \hline

 \multirow{5}{*}{PRAD-2000} & Bicubic& $\times4$ & &\underline{257.04}&\underline{14.19}&0.8045 &0.8177\\
 &BSRGAN& $\times4$ & &331.23&20.27&0.9029&0.8791\\ 
 &Real-ESRGAN& $\times4$ & & 300.24&14.83&0.8908&0.8994\\ 
 &SwinIR-GAN& $\times4$ & & 304.11&14.66&\underline{0.9308}&\underline{0.9308}\\\cline{2-8}
 &Ours& $\times4$ & &\textbf{220.96}&\textbf{11.77}&\textbf{0.9464}&\textbf{0.9467}\\\hline 
 \hline

\end{tabular}}
\label{table_full_no_0611}
\end{table*}

%% ablation study on different degradations (1st stage, realesrgan vs cdformer)
\begin{table*}[t]\small
\centering
\caption{ Comparisons of with and without stage 1 restoration module. The best and worst results are highlighted in \textbf{bold} and \textit{textit}. }
\label{table1}
\resizebox{0.98\textwidth}{!}{%
\begin{tabular}{c|c| c|c c c c c c c c c c |cc  }
\hline
\multirow{2}{*}{Datasets} & \multirow{2}{*}{Iterations} & \multirow{2}{*}{Degradation}  & \multicolumn{10}{c}{Metrics} & \multicolumn{2}{c}{Our Metrics}\\\cline{4-15} 
  & &  & & PSNR$\uparrow$ & SSIM$\uparrow$ &LPIPS$\downarrow$& ST-LPIPS$\downarrow$ & CLIP-IQA$\uparrow$ & MUSIQ$\uparrow$ &NIQE$\downarrow$ & BRISQUE$\downarrow$ & NRQM$\uparrow$& $L1_{texture}\downarrow$ & $L1_{intensity}\downarrow$ \\\hline
\hline
\multirow{8}{*}{PRAD-100} & \multirow{4}{*}{60k} &Real-ESRGAN without stage 1&  &24.70&0.5798&0.2417&0.2194& 0.4808&47.41&4.79&24.81&6.55 &255.63 &13.58\\ 
&&Real-ESRGAN with stage 1&  &24.67&0.5791&0.2415&0.2160&0.4769&47.51&4.92&25.39&6.66&245.92&13.15 \\
&&Codeformer without stage1&&24.75&0.5904&0.2369&0.2092&0.4712&46.44&4.69&26.93&6.57&235.52&12.30\\ 
&&Codeformer with stage 1&&24.72&0.5880&0.2362&0.2097&0.4454&44.57&4.88&29.65&6.46&\textbf{228.80}&\textbf{12.03}\\ 
 \cline{2-15}
 & \multirow{4}{*}{100k} &Real-ESRGAN without stage1&  &24.71&0.5802&0.2343&0.2079&0.4771&47.63&4.72&27.26&6.85&261.22 &14.04\\ 
 &&Real-ESRGAN with stage1&  &\textit{24.44}& \textit{0.5629} &\textit{0.2453} & 0.2138 &\textbf{0.4828} &\textbf{48.61}& \textbf{4.69}&\textbf{25.90}&\textbf{6.95}&270.34&14.80\\ 
&&Codeformer without stage1&  &25.19&0.6083&0.2384&0.2243&0.4361&42.65&5.03&30.47&6.07& 233.99&12.25\\ 
 &&Codeformer with stage1&  &24.89&0.6014&0.2280&\textbf{0.2022}&\textit{0.4365}&43.82&4.99&29.70&6.25&\textbf{209.50}&\textbf{11.46}\\ 
 \cline{2-15}
 & \multirow{4}{*}{160k} &Real-ESRGAN without stage1&  &24.70&0.5798&0.2299&0.2026&0.4813&47.88&4.69&26.96&6.79&236.14&12.86\\ 
 &&Real-ESRGAN with stage1&  &24.84& 0.5797 &0.2358 & 0.2156 &0.4731&47.31& 4.71&26.60&6.87&266.46&14.20\\ 
 &&Codeformer without stage1&  &25.15&0.6043&0.2368& 0.2216& 0.4378&43.39&4.77&29.12&6.26&241.85&12.47\\ 
&&Codeformer with stage1&  &\textbf{25.03}&\textbf{0.6081}&0.2287&0.2089&0.4439&\textit{43.49}&\textit{5.08}&30.93&\textit{6.16}&213.36&11.34\\ 
\cline{2-13}
% & \multirow{2}{*}{205k} &Real-ESRGAN&  &24.68&0.5741&0.2381&0.2126&0.4732&48.48&4.70&26.86&6.90\\ 
%  &&Codeformer&  &24.86&0.5947&\textbf{0.2279}&0.2079&0.4559&45.00&4.95&\textit{31.39}&6.34\\ 
 \hline \hline

\multirow{8}{*}{LUAD-100}& \multirow{4}{*}{60k}  &Real-ESRGAN without stage1& &25.42&0.6539&0.2443&0.2279&0.4178&44.33&5.19&30.17&5.30&215.91&14.83 \\ 
&&Real-ESRGAN with stage1&&24.41&0.6085&\textit{0.2972}&\textit{0.2497}&\textit{0.4042}&43.01&5.07&27.77&5.45&251.73&17.05 \\
& &Codeformer without stage1& &26.04&0.6878&0.2186&0.2073&0.4425&43.85&5.45&32.98&4.95&\textbf{187.61}&\textbf{12.46}\\ 
& &Codeformer with stage1& &25.79&0.6629&0.2674&0.2313&0.4134&\textit{41.50}&5.24&\textit{34.57}&4.96&188.37&13.17\\ 
\cline{2-15}
& \multirow{4}{*}{100k}  &Real-ESRGAN without stage1& &25.24&0.6465&0.2559&0.2130&0.4302&45.47&4.84&28.48&5.88& 228.60&15.33\\ 
&&Real-ESRGAN with stage1& &\textit{23.90}&\textit{0.5866}&0.2968&0.2472&0.4291&44.52&4.93&\textbf{26.06}&5.78&281.73&18.57\\ 
& &Codeformer without stage1&  &27.01&0.7181&0.2307&0.2429&0.3893&38.92&5.69&36.16&4.32& 193.67 &\textbf{12.61}\\
& &Codeformer with stage1&  &26.03&0.6785&0.2606&\textbf{0.2249}&0.4181&42.41&5.26&32.41&4.93&\textbf{182.38}&12.86\\ 
 \cline{2-15}
&\multirow{4}{*}{160k} &Real-ESRGAN without stage1& &25.31&0.6469&0.2568&0.2121&0.4468&46.16 &4.80&28.43
&5.81&211.31&14.14\\ 
&&Real-ESRGAN with stage1& &24.39&0.6013&0.2922&0.2368&0.4186&44.20&\textbf{4.78}&27.62&6.04&267.25&17.17\\
& &Codeformer without stage1&  &26.65&0.7041&0.2240&0.2213& 0.4124&41.48 &5.26&34.00
&4.85&191.67&12.46\\ 
& &Codeformer with stage1&  &\textbf{26.48}&\textbf{0.6935}&0.2576&0.2290&0.4133&41.61&\textit{5.33}&33.08&\textit{4.81}&176.38&12.64\\ 
 \cline{2-13} 
% &\multirow{2}{*}{205k} &Real-ESRGAN& &24.08&0.5902&0.2901&0.2307&0.4202&\textbf{45.77}&4.95&28.08&\textbf{6.09}\\ 
% & &Codeformer&  &25.92&0.6666&\textbf{0.2526}&0.2250&\textbf{0.4309}&43.22&5.12&33.14&5.15\\ 
 \hline \hline

\multirow{8}{*}{GBM-100}& \multirow{4}{*}{60k}  &Real-ESRGAN without stage1&  &22.79&0.4835&0.3031&0.3977&0.4863&49.62&5.34&25.13&6.07& 449.15& 24.12 \\ 
&&Real-ESRGAN with stage1&  &22.68&0.4768&0.3035&\textit{0.3826}&0.5027&51.58&5.26&25.48&6.17&388.25 & 22.00\\
& &Codeformer without stage1 &&23.25&0.5210&0.2837&0.3644&0.5018&50.50&5.16&27.29&5.94&\textbf{287.96}&16.30 \\
& &Codeformer with stage1 &&23.04&0.5087&0.2888&0.3675&0.4819&47.96&5.19&28.78&5.78&293.50&\textbf{15.01}\\ \cline{2-15} 
& \multirow{4}{*}{100k}  &Real-ESRGAN without stage1&  &22.79&0.4855&0.2975&0.3752&0.5025&50.99&5.09&25.74&6.45& 412.50&22.14\\ 
&&Real-ESRGAN with stage1&  &\textit{22.10}&\textit{0.4425}&\textit{0.3059}&0.3784&0.5115&52.53&4.92&21.70&6.70&492.34&26.22 \\ 
& &Codeformer without stage1&  &23.70&0.5471&0.3016&0.4039& 0.4639&45.42&5.74&32.82&5.01&277.43 &15.26\\
& &Codeformer with stage1&  &23.34&0.5357&0.2881&0.3628&0.4650&46.09&5.53&31.70&5.42&\textbf{231.49}&\textbf{12.51}\\ \cline{2-15}
&\multirow{4}{*}{160k} &Real-ESRGAN without stage1&  &22.55&0.4680&0.2816&0.3573&0.5153& 52.65&4.69&20.83&6.83&395.48&22.52 \\ 
 & &Real-ESRGAN with stage1&  &22.55&0.4617&0.2921&0.3784&0.5095&51.47&\textbf{4.53}&\textbf{20.84}&\textbf{6.93}&448.60&24.94\\ 
& &Codeformer without stage1&  &23.49&0.5292&0.2927&0.3790&0.4653&46.49&5.22&29.30&5.44&319.73&17.06 \\
& &Codeformer with stage1&  &23.25&0.5217&\textbf{0.2822}&0.3642&0.4767&47.39&5.05&28.36&5.85&272.71&14.06\\ \cline{2-13}
% &\multirow{2}{*}{205k} &Real-ESRGAN&  &22.41&0.4576&0.2988&0.3762&\textbf{0.5126}&\textbf{53.38}&4.77&21.75&6.74 \\ 
% & &Codeformer&  &22.88&0.4950&0.2894&0.3663&0.4862&49.13&4.94&27.52&5.96\\
\hline\hline
\end{tabular}}
\label{table_ablation_wostage1_0612}
\end{table*}
